Detecting Safety and Security Faults in PLC Systems with Data Provenance

Programmable Logic Controllers are an integral component for managing many different industrial processes (e.g., smart building management, power generation, water and wastewater management, and traffic control systems), and manufacturing and control industries (e.g., oil and natural gas, chemical, pharmaceutical, pulp and paper, food and beverage, automotive, and aerospace). Despite being used widely in many critical infrastructures, PLCs use protocols which make these control systems vulnerable to many common attacks, including man-in-the-middle attacks, denial of service attacks, and memory corruption attacks (e.g., array, stack, and heap overflows, integer overflows, and pointer corruption). In this paper, we propose PLC-PROV, a system for tracking the inputs and outputs of the control system to detect violations in the safety and security policies of the system. We consider a smart building as an example of a PLC-based system and show how PLC-PROV can be applied to ensure that the inputs and outputs are consistent with the intended safety and security policies.

==> Makefile <==
# "Improved" Makefile for LaTeX documents
# INTPUFILE This defines the name of the file you want to latex
# the make file will automatically look for INPUT.tex as the latex file
INPUTFILE:=plc-prov
LATEXCC:=

ifneq (, $(shell which latexrun))
  LATEXCC:=latexrun
else ifneq (, $(shell which latexmk))
  LATEXCC:=latexmk
endif

all:
ifeq ($(LATEXCC),pdflatex)
	pdflatex ${INPUTFILE}
	bibtex $(INPUTFILE)
	pdflatex ${INPUTFILE}
	pdflatex ${INPUTFILE}
else
	$(LATEXCC) $(INPUTFILE)
endif

view: ${INPUTFILE}.pdf
	open ${INPUTFILE}.pdf

${INPUTFILE}.pdf: all

.PHONY: open
open:
	@/Applications/Sublime\ Text.app/Contents/SharedSupport/bin/subl --project $(INPUTFILE).sublime-project

.PHONY: icloud
icloud: ${INPUTFILE}.pdf
	@cp ${INPUTFILE}.pdf ~/Library/Mobile\ Documents/com~apple~CloudDocs


